GGI Lectures on Exotic Hadrons

It is well known that M. Gell-Mann, introducing quarks in 1964 to describe the known mesons and baryons, hinted at the existence of further $qq\bar q\bar q$ mesons (tetraquarks) and $qqqq\bar q$ baryons (pentaquarks). In 1977, R. Jaffe proposed a model of the lightest scalar mesons as diquark-antidiquark pairs and A. de Rujula, H. Georgi and S. Glashow coined the term hadron molecules, to describe possible hadrons made by meson-antimeson pairs bound by the familiar nuclear forces, also an overall tetraquark system. The two alternative pictures have been employed to interpret the unexpected hadron discovered by Belle in 2003, the $X(3872)$, confirmed by BaBar and seen in many other High Energy experiments. Since then, a wealth of Exotic Hadrons have been discovered, mesons and baryons that cannot be described by the classical Gell-Mann, $q\bar q$ and $qqq$, configurations, opening a new chapter of Hadron Spectroscopy.

==> chapts/GGI_references.tex <==

\bibliographystyle{spphys}
\bibliography{quattro}
\begin{thebibliography}{99}%

\bibitem{GellMann:1964nj} M. Gell-Mann, {\it A Schematic Model of Baryons and Mesons}, PL {\bf 8},  214, 1964.
\bibitem{Olsen:2015zcy}
S.~L.~Olsen,
%``XYZ Meson Spectroscopy,''
PoS \textbf{Bormio2015} (2015), 050, [arXiv:1511.01589 [hep-ex]].

\bibitem{Belle:2011aa}
A.~Bondar \textit{et al.} [Belle],
%``Observation of two charged bottomonium-like resonances in Y(5S) decays,''
Phys. Rev. Lett. \textbf{108} (2012), 122001 [arXiv:1110.2251 [hep-ex]].

\bibitem{LHCb:2019kea}
R.~Aaij \textit{et al.} [LHCb],
%``Observation of a narrow pentaquark state, $P_c(4312)^+$, and of two-peak structure of the $P_c(4450)^+$,''
Phys. Rev. Lett. \textbf{122} (2019) no.22, 222001, [arXiv:1904.03947 [hep-ex]].

\bibitem{Tornqvist:1993ng}
N.~A.~Tornqvist,
%``From the deuteron to deusons, an analysis of deuteron - like meson meson bound states,''
Z. Phys. C \textbf{61} (1994), 525-537
doi:10.1007/BF01413192
[arXiv:hep-ph/9310247 [hep-ph]].

\bibitem{Guo:2017jvc}
F.~K.~Guo, C.~Hanhart, U.~G.~Mei\ss{}ner, Q.~Wang, Q.~Zhao and B.~S.~Zou,
%``Hadronic molecules,''
Rev. Mod. Phys. \textbf{90} (2018) no.1, 015004, [arXiv:1705.00141 [hep-ph]].

\bibitem{Maiani:2004vq}
L.~Maiani, F.~Piccinini, A.~D.~Polosa and V.~Riquer, Phys. Rev. D \textbf{71} (2005), 014028.

\bibitem{Dubynskiy:2008mq}
S.~Dubynskiy and M.~B.~Voloshin,
%``Hadro-Charmonium,''
Phys. Lett. B \textbf{666} (2008), 344-346, [arXiv:0803.2224 [hep-ph]].

\bibitem{Braaten:2014qka}
E.~Braaten, C.~Langmack and D.~H.~Smith,
%``Born-Oppenheimer Approximation for the XYZ Mesons,''
Phys. Rev. D \textbf{90} (2014) no.1, 014044, [arXiv:1402.0438 [hep-ph]].

\bibitem{book} A.~Ali, L.~Maiani and A.~D.~Polosa,  {\it Multiquark Hadrons}, Cambridge University Press (2019).

%@@@@@@@@@@@@@@@

\bibitem{Zeldovich:1967rt}
Y.~B.~Zeldovich and A.~D.~Sakharov,
%``Mass formulas for mesons and baryons in the quark model,''
Acta Phys. Hung. \textbf{22} (1967), 153-157.

\bibitem{DeRujula:1976zlg}
A.~De Rujula, H.~Georgi and S.~L.~Glashow, Phys. Rev. Lett. \textbf{38} (1977), 317.

\bibitem{Georgi:1982jb} H.~Georgi,
{\it Lie Algebras in Particle Physics. From Isospin to Unified Theories}, Front. Phys. \textbf{54} (1982), 1-255.

\bibitem{Zweig:1981pd} G. Zweig, G. {\it An SU(3) Model For Strong Interaction Symmetry And Its Breaking},
CERN-TH-412 (1974).

\bibitem{cole} S. Coleman, {\it Aspects of Symmetry: selected Erice lectures}, Cambridge University Press, 1985.

\bibitem{Gross:1973id} D.~J.~Gross and F.~Wilczek,
  %``Asymptotically Free Gauge Theories. 1,''
  Phys.\ Rev.\ {\bf  D 8} (1973) 3633;  %``Asymptotically Free Gauge Theories. 2.,''
  Phys.\ Rev.\  {\bf D 9} (1974) 980.

\bibitem{Politzer:1973fx} H.~D.~Politzer,
  %``Reliable Perturbative Results for Strong Interactions?,''
  Phys.\ Rev.\ Lett.\  {\bf 30} (1973) 1346.


%\cite{Karliner:2014gca}
\bibitem{Karliner:2014gca}
M.~Karliner and J.~L.~Rosner, Phys. Rev. D \textbf{90} (2014)094007
[arXiv:1408.5877 [hep-ph]].

%\cite{Karliner:2016zzc}
\bibitem{Karliner:2016zzc} M.~Karliner, S.~Nussinov and J.~L.~Rosner, Phys. Rev. D \textbf{95} (2017) no.3, 034011, [arXiv:1611.00348 [hep-ph]].

\bibitem{borgat} E. Borchi, R. Gatto, Phys. Lett. {\bf 14} (1965) 352.

\bibitem{jaf} R. Jaffe, Phys. Rev. {\bf D15} (1977) 267; R. Jaffe, F. Wilczek, Phys. Rev. Lett. {\bf 91} (2003) 232003. See also \cite{book}.

\bibitem{Maiani:2014aja} L. Maiani, F. Piccinini, A. D. Polosa and V. Riquer, Phys. Rev. {\bf D 89} (2014), 114010.

\bibitem{LHCb:2016axx} R.~Aaij \textit{et al.} [LHCb], Phys. Rev. Lett. \textbf{118} (2017) 022003, [arXiv:1606.07895 [hep-ex]].

\bibitem{Maiani:2016wlq} L. Maiani, A. Polosa, V. Riquer, Phys. Rev.  {\bf D 94} (2016) 054026.

\bibitem{lmaia16} L.Maiani, CERN, talk to the LHCb Collabration,  13/10/2016 and Shnghai, Jiao Tong Univerdity, 4/11/2016.

\bibitem{Esposito:2015fsa} A.~Esposito, A.~L.~Guerrieri, L.~Maiani, F.~Piccinini, A.~Pilloni, A.~D.~Polosa and V.~Riquer,
%``Observation of light nuclei at ALICE and the X(3872) conundrum,''
Phys. Rev. D \textbf{92} (2015) no.3, 034028, [arXiv:1508.00295 [hep-ph]].

\bibitem{BESIII:2020qkh}
M.~Ablikim \textit{et al.} [BESIII],
%``Observation of a Near-Threshold Structure in the $K^+$ Recoil-Mass Spectra in $e^+e^- \rightarrow K^+(D_s^-D^{*0}+D_s^{*-}D^0$),''
Phys. Rev. Lett. \textbf{126} (2021) no.10, 102001, [arXiv:2011.07855 [hep-ex]].

\bibitem{LHCb:2021uow}
R.~Aaij \textit{et al.} [LHCb],
%``Observation of New Resonances Decaying to $J/\psi K^+$+ and $J/\psi \phi$,''
Phys. Rev. Lett. \textbf{127} (2021) no.8, 082001, [arXiv:2103.01803 [hep-ex]].





\bibitem{mpr21} L. Maiani, A. D. Polosa and V. Riquer, Sci. Bull. {\bf 66} (2021), 1616, ArXiv:2103.08331.

\bibitem{glka} S. L. Glashow, R. H. Socolow, Phys. Rev. Letters {\bf 15} (1966) 329; mixing of two Kaons belonging to different nonets is considered  in G. L. Kane, Phys. Rev. {\bf 156} (1967) 1738.

\bibitem{Bedolla:2019zwg} M.~A.~Bedolla, J.~Ferretti, C.~D.~Roberts and E.~Santopinto,
%``Spectrum of fully-heavy tetraquarks from a diquark+antidiquark perspective,''
Eur. Phys. J. C \textbf{80} (2020) no.11, 1004, [arXiv:1911.00960 [hep-ph]].

\bibitem{Becchi:2020uvq} C.~Becchi, J.~Ferretti, A.~Giachino, L.~Maiani and E.~Santopinto,
%``A study of $c c\bar{c}\bar{c}$ tetraquark decays in 4 muons and in $D^{(*)} \bar{D}^{(*)}$ at LHC,''
Phys. Lett. B \textbf{811} (2020), 135952, [arXiv:2006.14388 [hep-ph]].

\bibitem{Das:1967it} T.~Das, G.~S.~Guralnik, V.~S.~Mathur, F.~E.~Low and J.~E.~Young,
%``Electromagnetic mass difference of pions,''
Phys. Rev. Lett. \textbf{18} (1967), 759-761.

\bibitem{colgla} S. Coleman, S. L. Glashow, Phys. Rev.  {\bf 134} (1964) 1367. 

\bibitem{Gasser:1974wd} J.~Gasser and H.~Leutwyler,
%``Implications of Scaling for the Proton - Neutron Mass - Difference,''
Nucl. Phys. B \textbf{94} (1975), 269.

\bibitem{njl} Y. Nambu, G. Jona-Lasinio, Phys. Rev. {\bf 122} (1961) 345; Y. Nambu, G. Jona-Lasinio, Phys. Rev. {\bf 124}
  (1961) 246.

\bibitem{gmor} M. Gell-Mann, R. Oakes and J. Renner, Phys. Rev. {\bf 175} (1968) 2195.

\bibitem{glwe} S. L. Glashow and S. Weinberg, Phys. Rev. Letters {\bf 20} (1968) 224.

\bibitem{Dashen:1969eg} R. Dashen, Phys. Rev. {\bf 183}  (1969) 1245.

\bibitem{cm70}  N. Cabibbo, L. Maiani,in  {\it Evolution of Particle Physics. }A Volume Dedicated to Edoardo Amaldi on his Sixtieth Birthday. M. Conversi (editor), Academic Press (1970).


\bibitem{Karliner:2017gml}
M.~Karliner and J.~L.~Rosner,
%``Isospin splittings in baryons with two heavy quarks,''
Phys. Rev. D \textbf{96} (2017) no.3, 033004, [arXiv:1706.06961 [hep-ph]].

\bibitem{Maiani:2017kyi} L. Maiani, A. D. Polosa and V. Riquer, Phys. Lett. {\bf B 778} (2018) 247.


\bibitem{Selem:2006nd}
A.~Selem and F.~Wilczek,
%``Hadron systematics and emergent diquarks,''
[arXiv:hep-ph/0602128 [hep-ph]].

\bibitem{mpr20} L. Maiani, A. D. Polosa and V. Riquer, Phys. Rev. {\bf D 102} (2020) 034017.

\bibitem{lhcb21} LHCb Collaboration, Lepton Photon Conference 2021.

\bibitem{lhcb18} R. Aaij \textit{et al.} [LHCb], Phys. Rev. Lett. \textbf{121} (2018) 162002.


\bibitem{Karliner:2017qjm}
M.~Karliner and J.~L.~Rosner,
%``Discovery of doubly-charmed $\Xi_{cc}$ baryon implies a stable ($b b \bar{u} \bar{d}$) tetraquark,''
Phys. Rev. Lett. \textbf{119} (2017) no.20, 202001, [arXiv:1707.07666 [hep-ph]]. 


\bibitem{Eichten:2017ffp}
E.~J.~Eichten and C.~Quigg,
%``Heavy-quark symmetry implies stable heavy tetraquark mesons $Q_iQ_j \bar q_k \bar q_l$,''
Phys. Rev. Lett. \textbf{119} (2017) no.20, 202002
[arXiv:1707.09575 [hep-ph]].

\bibitem{hbhq} M. Savage, M. B. Wise, Phys. Lettters \textbf{B 248} (1990) 177; N. Brambilla, A. Vairo and T. Rosch, Phys. Rev. \textbf{D 72} (2005) 034021; for recent applications see T. Mehen, Phys. Rev. \textbf{D 96} (2017) 09402, [arXiv:1708.05020 [hep-ph]].


\bibitem{weqm} see: S. Weinberg, {\it  Lectures on Quantum Mechanics}, Cambridge University Press (2015).

\bibitem{pauling} A standard reference on $H,~H_2$ and $He$ molecules and ions is L. Pauling and E. B. Wilson Jr., {\it Introduction to Quantum Mechanics with Applications to Chemistry}. Dover Books on Physics (1985).

\bibitem{mpr19} Explicit derivations are found in L. Maiani, A. D.Polosa and V. Riquer, Phys. Rev.  {\bf D100} (2019) 074002, arXiv:1908.03244.

\bibitem{Bali:2000gf}
G.~S.~Bali,
%``QCD forces and heavy quark bound states,''
Phys. Rept. \textbf{343} (2001), 1-136, [arXiv:hep-ph/0001312 [hep-ph]].

\bibitem{Karliner:2014gca}
M.~Karliner and J.~L.~Rosner,
%``Baryons with two heavy quarks: Masses, production, decays, and detection,''
Phys. Rev. D \textbf{90} (2014) no.9, 094007, [arXiv:1408.5877 [hep-ph]].

\bibitem{Mathur:2018rwu}
N.~Mathur and M.~Padmanath,
%``Lattice QCD study of doubly-charmed strange baryons,''
Phys. Rev. D \textbf{99} (2019) no.3, 031501, [arXiv:1807.00174 [hep-lat]].

\bibitem{LHCb:2018pcs}
R.~Aaij \textit{et al.} [LHCb],
%``First Observation of the Doubly Charmed Baryon Decay $\Xi_{cc}^{++}\rightarrow \Xi_{c}^{+}\pi^{+}$,''
Phys. Rev. Lett. \textbf{121} (2018) no.16, 162002, [arXiv:1807.01919 [hep-ex]].
\bibitem{Esposito:2013fma} A. Esposito, M. Papinutto, A. Pilloni, A. D. Polosa, and N. Tantalo, Phys. Rev. {\bf D88}, 054029 (2013). 
\bibitem{Karliner:2017qjm}
M.~Karliner and J.~L.~Rosner,
%``Discovery of doubly-charmed $\Xi_{cc}$ baryon implies a stable ($b b \bar{u} \bar{d}$) tetraquark,''
Phys. Rev. Lett. \textbf{119} (2017) no.20, 202001, [arXiv:1707.07666 [hep-ph]].

\bibitem{Eichten:2017ffp}
E.~J.~Eichten and C.~Quigg,
%``Heavy-quark symmetry implies stable heavy tetraquark mesons $Q_iQ_j \bar q_k \bar q_l$,''
Phys. Rev. Lett. \textbf{119} (2017) no.20, 202002, [arXiv:1707.09575 [hep-ph]].

\bibitem{Luo:2017eub}
S.~Q.~Luo, K.~Chen, X.~Liu, Y.~R.~Liu and S.~L.~Zhu,
%``Exotic tetraquark states with the $qq\bar{Q}\bar{Q}$ configuration,''
Eur. Phys. J. C \textbf{77} (2017) no.10, 709, [arXiv:1707.01180 [hep-ph]].

\bibitem{lattice19} P.  Junnarkar  et al., Phys.\ Rev.\ D {\bf 99} (2019) 034507;   A. Francis {\it et al.},
Phys.\ Rev.\ D {\bf 99} (2019), Phys. Rev. Lett. \textbf{118} (2017) 142001, 014002 (2019);  L.~Leskovec, S.~Meinel, M.~Pflaumer and M.~Wagner,  Phys.\ Rev.\ D {\bf 100} (2019) 014503.

\bibitem{hooftN} G.~'t Hooft,~Nucl.~Phys. {\bf B72}~(1974)~461;~Comm.~Math.~Phys.~{\bf 88} (1983) 1.

\bibitem{Witten:1979kh} E. Witten, Nucl. Phys. {\bf B 160} (1979) 57.

\bibitem{duality} Dolen, D.~Horn and C.~Schmid,  Phys.\ Rev.\ Lett.\  {\bf 19}  (1967), 402; Phys.\ Rev.\  {\bf 166} (1968), 1768. 

\bibitem{Veneziano:1968yb} G. Veneziano, Nuovo Cim. {\bf A57} (1968) 190.

\bibitem{duality2} M. B. Green, J. H. Schwarz and E. Witten, {\it Superstring Theory}, Vol. 1, Cambridge University Press (2012).

\bibitem{Weinberg:2013cfa} S. Weinberg, Phys. Rev. Letters {\bf 110} (2013) 261601.

\bibitem{knepar} M. Knecht and S. Peris, Phys. Rev. {\bf D 88} (2013) 036016, arXiv:1307.1273.

\bibitem{cohen} Cohen, Phys. Rev. {\bf D 89} (2014) 054018; 1403.8090.

\bibitem{handle1} T. Cohen and R. Lebed, Phys. Rev. {\bf D 90} (2014) 016001, arXiv 1403.8090; L. Maiani, A. D. Polosa and V. Riquer, JHEP 1606 (2016) 160.

\bibitem{Maiani:2018pef} L. Maiani, A.D. Polosa, V. Riquer, Phys. Rev. {\bf D 98} (2018) 054023.

\bibitem{rosven16} G.~C.~Rossi and G.~Veneziano, Nucl.\ Phys.\ B {\bf 123} (1977) 507; JHEP {\bf 06} 041 (2016) and references therein.

\bibitem{mrw18} L. Maiani, V. Riquer and W. Wang, Eur. Phys. J. {\bf C 78} (2018) 1011.x

\bibitem{Cotugno:2009ys}
G.~Cotugno, R.~Faccini, A.~D.~Polosa and C.~Sabelli,
%``Charmed Baryonium,''
Phys. Rev. Lett. \textbf{104} (2010), 132005 [arXiv:0911.2178 [hep-ph]].



\bibitem{Weinberg:1965zz}
S.~Weinberg,
%``Evidence That the Deuteron Is Not an Elementary Particle,''
Phys. Rev. \textbf{137} (1965), B672-B678.

\bibitem{Workman:2022}
R.L.~Workman \textit{et al.} [Particle Data Group],
%``Review of Particle Physics,''
to be published (2022), 

\bibitem{Esposito:2021vhu} A.~Esposito, L.~Maiani, A.~Pilloni, A.~D.~Polosa and V.~Riquer,
%``From the line shape of the X(3872) to its structure,''
Phys. Rev. D \textbf{105} (2022) no.3, L031503, [arXiv:2108.11413 [hep-ph]].

\bibitem{weinb05} see, e.g., S. Weinberg, {\it The Quantum theory of fields}, Vol. 1. Cambridge University Press (2005).

\bibitem{landasmor} Ya. A. Smorodinsky, Dokl.Akad.Nauk SSSR {\bf 60} (1948) 217;  L. D. Landau and  E. M. Lifshitz, {\it Quantum Mechanics}, Vol. 3, \S 133, Problem 1, Butterworth (2003); we follow here: H. A. Bethe, Phys.Rev. {\bf 76} (1949) 38.

\bibitem{LHCb:2021auc}
R.~Aaij \textit{et al.} [LHCb],
%``Study of the doubly charmed tetraquark $T_{cc}^+$,''
[arXiv:2109.01056 [hep-ex]].

\bibitem{Baru:2021ldu}
V.~Baru, X.~K.~Dong, M.~L.~Du, A.~Filin, F.~K.~Guo, C.~Hanhart, A.~Nefediev, J.~Nieves and Q.~Wang,
%``Effective range expansion for narrow near-threshold resonances,''
[arXiv:2110.07484 [hep-ph]].

\bibitem{Esposito:2013fma}
A.~Esposito, M.~Papinutto, A.~Pilloni, A.~D.~Polosa and N.~Tantalo,
%``Doubly charmed tetraquarks in $B_c$ and $\Xi_{bc}$ decays,''
Phys. Rev. D \textbf{88} (2013) no.5, 054029, [arXiv:1307.2873 [hep-ph]]

\bibitem{Mikhasenko:2022rrl}
M.~Mikhasenko,
%``Effective-range expansion of the $T_{cc}^+$ state at the complex $D^{*+}D^0$ threshold,''
[arXiv:2203.04622 [hep-ph]].

\end{thebibliography}

